Enabling Efficient Dynamic Resizing of Large DRAM Caches via A Hardware Consistent Hashing Mechanism

Die-stacked DRAM has been proposed for use as a large, high-bandwidth, last-level cache with hundreds or thousands of megabytes of capacity. Not all workloads (or phases) can productively utilize this much cache space, however. Unfortunately, the unused (or under-used) cache continues to consume power due to leakage in the peripheral circuitry and periodic DRAM refresh. Dynamically adjusting the available DRAM cache capacity could largely eliminate this energy overhead. However, the current proposed DRAM cache organization introduces new challenges for dynamic cache resizing. The organization differs from a conventional SRAM cache organization because it places entire cache sets and their tags within a single bank to reduce on-chip area and power overhead. Hence, resizing a DRAM cache requires remapping sets from the powered-down banks to active banks. In this paper, we propose CRUNCH (Cache Resizing Using Native Consistent Hashing), a hardware data remapping scheme inspired by consistent hashing, an algorithm originally proposed to uniformly and dynamically distribute Internet traffic across a changing population of web servers. CRUNCH provides a load-balanced remapping of data from the powered-down banks alone to the active banks, without requiring sets from all banks to be remapped, unlike naive schemes to achieve load balancing. CRUNCH remaps only sets from the powered-down banks, so it achieves this load balancing with low bank power-up/down transition latencies. CRUNCH's combination of good load balancing and low transition latencies provides a substrate to enable efficient DRAM cache resizing.

==> Makefile <==
all: paper.pdf

nobib: $(wildcard *.tex secs/*.tex figs/*.pdf figs/*.png)
	pdflatex paper

paper.bbl: paper.bib
	pdflatex paper
	bibtex paper

paper.pdf: $(wildcard *.tex secs/*.tex figs/*.pdf figs/*.png) paper.bbl
	pdflatex paper
	pdflatex paper

# For a re-run of latex (e.g., if there are unresolved references)
force:
	pdflatex paper
again: force

# Force a re-run of bibtex
bibtex:
	touch paper.bib
	pdflatex paper
	bibtex paper

wc: paper.pdf
	./wordcount.pl

clean:
	-rm -f paper.aux paper.log paper.blg paper.brf paper.dvi paper.txt paper.pdf

show: paper.pdf
	xpdf paper.pdf

# This is just for Gabe running on Cygwin/Windows
once: $(wildcard *.tex secs/*.tex figs/*.pdf figs/*.png) paper.bbl
	pdflatex paper
show2: paper.pdf
	- /cygdrive/c/Program\ Files/Adobe/Reader\ 10.0/Reader/AcroRd32.exe /n /s /A "pagemode=none" paper.pdf


==> secs/hpca-power-impact.tex <==
\subsection{Performance of Bank Utility Predictor}
\label{sec:bup-eval}
In \ssecref{bup}, we stated that the goal of our bank utility predictor (called
BUP for short) is to achieve performance within 5\% of having all banks enabled.
\figref{predictor.pdf} shows the comparison between BUP's predicted number of
banks and the minimum bank numbers which stay within 5\% of performance (labeled
$B_{5}\%$). The minimum bank numbers are determined by exhaustive search for
each workload. In addition, \figref{bup-norm-ipc.pdf} shows the performance of
each workload with the predicted bank count, normalized to the all banks enabled
case.

The data shows that BUP successfully predicts the exhaustively determined
value for seven workloads. The BUP scheme over-predicts the number of
required banks for WL-4, which is more acceptable behavior from the performance
perspective, since the performance remains within the 5\% target. However, BUP
misses opportunities to reduce DRAM cache power consumption in this case. On the
other hand, the BUP scheme under-predicts for WL-1 and WL-2, which further
reduces DRAM cache power consumption by 10\% and 18\% compared to using the
$B_{5}\%$ at the cost of degrading performance by 10.8\% and 7.5\%,
respectively.

We also observe that WL-10, which consists four copies of \texttt{gcc}, does not
benefit from using the DRAM cache, having less than 1\% performance degradation
without using the DRAM cache. This is because \texttt{gcc} has \emph{very low}
memory intensity (<2 L3-MPKI). Having extra cache capacity and bandwidth
provides minimal performance improvement for this workload.  Due to this
observation, BUP identifies very low memory-intensity application by monitoring
applications' MPKI values over time. If the total MPKI is less than a very low
threshold, $5$ in our experiments, BUP makes the decision to shut down the
entire DRAM cache.

%\todo{I think what we can do here is for each workload, run it once to see what the predicted
%number of banks to enable should be, then run it again with that number of banks statically
%enabled.  Then show the performance compared to having all banks enabled (ideally, we should be
%able to turn off quite a few banks with minimal performance impact).  Perhaps have another
%graph (or instead of performance) that just shows the ideal number of banks from the working-set
%size analysis, and then shows how many we predict.}

\figputT{predictor.pdf}{0in 0in 0in 0in}{Accuracy of the bank utility predictor.}
\figputT{bup-norm-ipc.pdf}{0in 0in 0in 0in}{System performance of the bank
utility predictor.}

\subsection{Power Impacts} To quantify the impacts of our DRAM cache power
management, we used the modified Micron power calculator to model both the DRAM
cache and off-chip DRAM. \figref{DRAM_cache_power_breakdown.pdf} plots the
breakdown of the DRAM cache power with all eight banks enabled. It is clear that
the static power (i.e., "Background" and "Refresh") dominates the total DRAM
cache power, much of which is contributed by the background power. When DRAM
cache accesses are less frequent, as in the case of WL-10, background power
alone consumes 83\% of the total power. By shutting off banks, we can linearly
scale down the large static power, leading to reductions in the total DRAM cache
power.

Note that the activation power is much smaller than the read/write (RD/WR)
power. This is due to the larger data width (64 bits) of the DRAM cache compared
to a traditional DRAM's as explained in \secref{meth}. As a result, each
activation command activates a single DRAM chip as opposed to eight in x8 DDR3.

\figref{DRAM_cache_power_sensitivity.pdf} shows DRAM cache power sensitivity to
varying number of enabled banks. Each bar in a cluster represents active bank
count, which ranges from eight to one from left to right, normalized to the
eight-bank configuration. The bars are further broken down into background power
and remaining DRAM cache power ("Others"). As expected, we can gain almost
linear power savings (63-79\%) with fewer active banks. Most of the power
savings come from background power, which scales linearly. The dynamic power, on
the other hand, remains roughly the same because the number of reads and writes
to the DRAM cache are constant to the first order.

\figputT{DRAM_cache_power_breakdown.pdf}{0in 0.6in 0in 1.4in}{Breakdown of DRAM
cache power with all eight banks enabled.}
\figputT{DRAM_cache_power_sensitivity.pdf}{0in 1.5in 0in 1.5in}{DRAM cache power
sensitivity to varying number of banks enabled.}

The power impacts of bank shutdown are best understood in the context of memory
system power, which \figref{Memory_system}(a) presents. Again, each bar in a
cluster represents the number of active banks in the DRAM cache. With only one
bank enabled, the total memory system power reduces by 12-23\%. This reduction
is achieved despite the slight increase in the off-chip DRAM power caused by the
extra traffic from increased DRAM cache misses. In other words, the significant
reduction in the DRAM cache power offsets the higher off-chip DRAM power,
resulting in net power savings.

Nonetheless, the power reductions must be weighed against performance.
\figref{Memory_system}(b) plots the corresponding performance of CRUNCH. The
highlighted bars indicate the minimum bank count using the 5\% performance
target used in the previous section. By varying the threshold of BUP, we can
make different power-performance trade-offs. Future work includes dynamically
adjusting the threshold based on working conditions and available power budgets.

\begin{figure}
\begin{center}
\begin{tabular}{c}
\hspace{-0.35in} \includegraphics[trim=0in 0in 0in 0.0in, clip, width=1.0\linewidth]{plots/Memory_system_power_breakdown} \\ {\footnotesize\sf\bfseries (a)} \\[-0.2in]
\hspace{-0.3in}\includegraphics[trim=0in 3in 0in 0in, clip, width=1.1\linewidth]{plots/crunch_ipc} \\[-0.1in] {\footnotesize\sf\bfseries (b)}
\end{tabular}
\caption{(a) The Impact of bank shut-down with CRUNCH on the memory system
power, and (b) the corresponding performance (dark bar indicates the fewest
banks enabled with no more than a 5\% slowdown compared to all banks
enabled).\label{fig:Memory_system}} \end{center}
\end{figure}




==> secs/model.tex <==
\subsection{An Analytical Model to Study the Impact on Performance
and Energy of Different Mapping Schemes}
Our evaluations, so far, have decoupled and analyzed the impact of
using different data mapping schemes, on steady-state and
transient performance/energy. The reason, for this decoupling, as
we described in Section~\ref{sec:meth}, is that performing full scale
simulations to quantify the impact of different mapping schemes on performance
and energy would require prohibitively long simulation time. In this section, we
attempt to capture the overall performance and energy trends using an analytical
model.

%in order to perform full scale
%simulations that to quantify the impact of different mapping
%schemes on performance and energy, we would have to run long,
%time-consuming simulations. In this section, we attempt to capture
%the overall performance and energy trends using an analytical
%model.

Please note that we do {\em not} intend this model as a
replacement for full-blown simulations. In order to simplify the
model, we make several assumptions, as we will detail below,
potentially introducing inaccuracies in our performance and energy
numbers. However, we believe that our model can help understand the overall
performance/energy trends for different data mapping policies, at
a high level.

%
%\figputW{isca/model-time-crop}{0in 0in 0in 0in}{Performance of mapping schemes
%with different bank configurations ($b$).}
%\figputT{isca/model-time-crop}{0in 0in 0in 0in}{Different Steady State Configurations.}
\begin{figure*}[t]
\begin{minipage}{\linewidth}
\footnotesize
\begin{center}
%\includegraphics[clip,scale=0.5]{plots/isca/model-time-crop}
\includegraphics[clip,height=4cm]{plots/isca/model-time-crop}
\end{center}
\caption{Performance of mapping schemes with different bank configurations ($b$).
\label{fig:isca/model-time-crop}}
\end{minipage}
\end{figure*}
%

\noindent
\textbf{Performance Model:}\\
First, we will present our model for performance. Our model uses
the execution time (in cycles) metric to quantify performance.
Execution time is composed of two major components: i) \mbox{steady-state} execution time and ii) transition time.

In order to compute steady-state execution time, we fix the amount
of work done - number of instructions retired (${N}$) - in steady
state and compute the execution time as a function of the number
of instructions retired and IPC (Instructions retired per cycle).

In order to factor in the time spent in transitions, we assume
that we transition at regular intervals (at a given frequency)
between keeping $b$ banks and $8$ banks powered on. We add the
amount of time spent in doing bank power-down/up transitions, to
the steady-state execution time. We express the transition time as
a function of the number of transitions and the time for each
transition.
\begin{equation}
\begin{multlined}
\textrm{Execution Time} = \frac{N}{2 \times IPC(8)} + \frac{N}{2
\times IPC(b)}\\ + M_{Up} \times T_{Up}(8-b) + M_{Down} \times
T_{Down}(8-b)
\end{multlined}
\end{equation}
\noindent where\\
$N$ - number of instructions retired in steady state\\
$b$ - number of powered up banks in steady state\\
$IPC(8)$ - steady-state IPC with 8 banks powered on\\
$IPC(b)$ - steady-state IPC with b banks powered on\\
$M_{Up}$ - number of power up transitions\\
$M_{Down}$ - number of power down transitions\\
$T_{Up}(8-b)$ - power-up transition latency to turn on $(8-b)$
banks (we transition from 8 to $b$ banks)\\
$T_{Down}(8-b)$ - power-down transition latency to turn off $(8-b)$
banks (we transition from $b$ to 8 banks)\\

\noindent
We use average results (across all workloads) from our steady
state and transient analysis simulations for $IPC(8)$, $IPC(b)$,
$T_{Up}(8-b)$ and $T_{Down}(8-b)$, for different mapping
schemes.\\

\noindent
We assume the same number of up and down transitions ($M_{Up}$ and
$M_{Down}$). This is a function of the transition frequency,
expressed in terms of \emph{Transitions per Million Instructions (TPMI)}.

$M_{Up} = M_{Down} = \frac{N (\textrm{in Million Instructions})}{TPMI
(\textrm{Transitions per Million Instructions)}}$

\noindent
We assume the same $M_{Up}$ and $M_{Down}$ for all mapping
schemes. This is a valid assumption, since we fix total number of
instructions retired ($N$) for all mapping schemes and express the
transition frequency in terms of Transitions per million
instructions ($TPMI$).

\figref{isca/model-time-crop} shows the execution time from
our model for BFO, MRI and CRUNCH, with varying transition
frequency ($TPMI$), for different values of b. First, when $b$ is
1, CRUNCH degrades performance as compared to both BFO and MRI, as
the transition frequency is increased. This is because CRUNCH has
similar steady-state performance as BFO and MRI, but has slightly higher
transition latencies than BFO and MRI, since cache sets in all the
7 turned-off banks need to be remapped. However, as the value of
$b$ is increased, CRUNCH outperforms BFO and MRI, since it has
better steady-state performance than both BFO and MRI, and lower
transition latencies than MRI. We observe a similar trend for
other values of $b$ as well.  Therefore, we conclude that CRUNCH is
effective in providing better system performance overall.

\noindent
\textbf{Energy Model:}\\
We model energy along similar lines as our performance model. We do not present
our energy model and results due to space constraints. However, the trends are
similar to our results from the performance model, as expected. CRUNCH provides
lower overall energy consumption than both BFO and MRI.

\ignore{

Our energy model is along similar lines as our performance model.
We express energy as a function of steady state energy consumption
and transition energy consumption.

Steady state energy consumption is expressed as the steady state
execution multiplied by the power expended each cycle.

Transition energy consumption is expressed as the number of
transitions times energy expended for each transition.

\begin{equation}
\begin{multlined}
\textrm{Energy} = \frac{N}{2 \times IPC(8)} \times P(8) + \frac{N}{2
\times IPC(b)} \times P(b)\\ + M_{Up} \times E_{Up}(8-b) + M_{Down} \times
E_{Down}(8-b)
\end{multlined}
\end{equation}


\noindent where\\
$N$ - number of instructions retired in steady state\\
$b$ - number of powered up banks in steady state\\
$IPC(8)$ - steady state instructions retired per cycle (IPC) when 8 banks
are powered on\\
$IPC(b)$ - steady state instructions retired per cycle (IPC) when b banks
are powered on\\
$P(8)$ - steady state power when 8 banks are turned on\\
$P(b)$ - steady state power when b banks are turned on\\
$M_{Up}$ - number of power up transitions\\
$M_{Down}$ - number of power down transitions\\
$E_{Up}(8-b)$ - power up transition energy to turn on $(8-b)$
banks (we transition from 8 to $b$ banks)\\
$E_{Down}(8-b)$ - power down transition energy to turn off $(8-b)$
banks (we transition from $b$ to 8 banks)\\

\noindent
We use average results (across all workloads) from our steady
state and transient analysis simulations for $IPC(8)$, $IPC(b)$,
$P(8)$, $P(b)$, $E_{Up}(8-b)$ and $E_{Down}(8-b)$, for different
mapping schemes.\\

\noindent
Our other assumptions are the same as those we make for our
performance model.

}


==> secs/old-related.tex <==
\section{Related Work}
\label{sec:related}

There is a significant body of prior work in cache power savings techniques that
take advantage of the dynamic nature of cache utilization.  Selectively
disabling ways in the L1 data cache has been proposed to save power using a
number of techniques to deal with modified data from flushing it to the L2
cache, to having special mechanisms to manage coherence and accesses to
modified data in disabled ways~\cite{Albonesi:Micro99}.  Our work focuses on a
large DRAM cache where shutting down ways is not practical and a re-indexing
scheme is required to deal with bank shutdown.  In addition, our shutdown
mechanism saves on leakage power whereas the previous
work~\cite{Albonesi:Micro99} only discusses dynamic power savings.

A number of academic papers have dealt with \kevin{need to double check if they
all do bank shut down}bank shutdown for leakage power
savings~\cite{Albonesi:Micro99,Bardine:CompArch,Golubeva:ISLPED07,
Li:DATE04,Powell:ISLPED00,zhang-isca2003}.
Other works have proposed reducing leakage in SRAM structures through a
Gated-Vdd mechanism and powering down ways of the
cache~\cite{Powell:ISLPED00,Golubeva:ISLPED07}, as well as expanding this
concept to dynamically gate ways of D-NUCA caches~\cite{Bardine:CompArch}.

Li et al.~examined the tradeoffs between different cache leakage reduction
techniques~\cite{Li:DATE04}, while Abella et al.  considered hardware techniques
to dynamically adapt the cache size to the program requirements by disabling
cache lines deemed unlikely to be resumed~\cite{Abella:TACO05}.

Yang et al.~\cite{yang-hpca2001} propose dynamically resizing I-caches to save
leakage power. Their DRI I-cache proposal monitors miss rate on an interval
basis and resizes the I-cache by comparing the measured miss rate to a preset
threshold. Similar to resizing DRAM caches, their resizing mechanism also
changes the number of active cache sets. However, they only allow power-of-two
resizing in order to address the indexing issue using a simple scheme that
changes the number of set index bits from the lookup address for mapping sets,
which achieves the same effect as MRI. Since their mechanism does not
consider dirty cache lines, it is not applicable to DRAM caches. In addition,
Their mechanism is orthogonal to \titleShort
because it focuses on a policy to determine how many sets to dynamically resized.
\kevin{Might be too verbose.}
%In addition, their mechanism does not
%consider dirty cache lines, thus there is no transition overhead from migrating
%or writing back dirty cache lines. Their mechanism is orthogonal to \titleShort
%because it focuses on a policy to determine how many sets to dynamically resized.

Industry processors have also adapted dynamic cache sizing techniques for
leakage power reduction. The Intel Core Duo Processor~\cite{Naveh:2006}
implemented a dynamically sizeable L2 cache which is sized to be small upon
wakeup from a deep sleep state. Similarly, AMD's Steamroller
processor~\cite{SteamRoller} also implements resizing of the L2 cache based on
the workload.  Both of these implementations disable ways of the cache to
achieve a smaller size. This paper builds on the concept of dynamically sizing
caches for application needs. However, unlike previous work that examines
gating small SRAM cache structures by disabling ways, we apply dynamic sizing to
large DRAM structures where the only viable option to resizing the cache
requires a re-indexing scheme.

\todo{~\cite{Abella:TACO05}. Abella's work is actually on powering down "lines" not banks!}

\todo{Talk about prior works on resizing policies (e.g., determining number of
shutdown banks and frequencies).}

There has also been significant work in reducing power in off-chip
DRAMs~\cite{Cooper:Micro10,Delaluz:HPCA01,Hur:HPCA08,Udipi:ISCA10}.  However,
these papers focus on reducing DRAM power when DRAMs are used for memory via
techniques such as partial activation of the DRAM array or low energy operating
modes and do not address the issue of using the DRAM as a cache and disabling
portions of the cache.  To the best of our knowledge, we are the first to
address bank shutdown policies in a stacked DRAM cache and address the
implementation constraints that require re-indexing schemes.



==> secs/pattern.tex <==
\section{Experimental Methodology}
\label{sec:meth}

\begin{table*}[t]
\centering
\footnotesize{
\begin{tabular}{|l||l|}
\hline
\textbf{Parameter} & \textbf{Setting} \\
\hline
\hline
Processor & 4-core, 3.2 GHz, Out-of-order, 4-wide issue, 256 ROB\\
\hline
Private L1 cache & 4-way associative, 32 KB \\
\hline
Shared L2 cache & 16-way associative, 4 MB\\
\hline
\hline
Stacked DRAM cache & 128 MB, 1 GHz (DDR 2 GHz), 128-bit channel,
channels/ranks/banks = 4/1/8, 2 KB rows, tCAS/tRCD/tRP = 8/8/15 \\
\hline
Off-chip DRAM & 8 GB, 800 MHz (DDR3 1.6 GHz~\cite{micronDDR3_4Gb}),
64-bit channel, channels/ranks/banks = 2/1/8, 2 KB rows, tCAS/tRCD/tRP =
11/11/11 \\
\hline
\end{tabular}
}
\vspace{-0.05in}
\caption{Simulated system parameters.}
\label{table:sysparams}
\end{table*}

\noindent\textbf{Simulator model:}
We use MacSim~\cite{macsim}, a cycle-level x86 CMP simulator for our evaluations of
application-level performance. We model a quad-core CMP systems with private L1
caches, and a shared L2 cache. We use a detailed DRAM
timing model for the shared L3 \emph{stacked DRAM} cache and the off-chip main
memory (DDR3 SDRAM-1600~\cite{micronDDR3_4Gb}).  Unless stated otherwise, our
detailed system configuration is as shown in Table~\ref{table:sysparams}.

\noindent\textbf{Power model:}
\kevin{Yasuko, can you update this subsection based on the new parameters you
decided to use at the end?}
We modified Micron's DRAM power calculator~\cite{micron-tr} to estimate stacked
DRAM cache power. In contrast to off-chip DDR3, stacked DRAM has a much wider
data width of 64 bits. Hence, only one stacked DRAM chip needs to be accessed
for each read or write command, as opposed to eight chips in a case of x8 DDR3.
This in turn indicates that stacked DRAM requires less activation energy for
each activation command, although we assume the actual read/write energy itself
remains the same because the same total number of bits are driven.

We adjust the IDD values extracted from the x8 DDR3-1600 datasheet
~\cite{micron-ds4251} as explained above. Furthermore, we double stacked DRAM's
refresh rate to factor in the higher operating temperature
~\cite{ghosh-micro2007}.

\noindent\textbf{Workloads:}
We evaluate our system using benchmarks drawn from SPEC CPU2006~\cite{spec}. We
mainly focus on high memory-intensity benchmarks for our main evaluations since
using DRAM cache has very little performance impact on low memory-intensity benchmarks.
In order to form suitable workloads, we split the benchmarks based on L2 misses
per thousand instructions (MPKI). Benchmarks with MPKI > 25 are in Category H
(high intensity), while the remaining with MPKI > 15 is in Category M (medium
intensity), and the rest of benchmarks is in Category L (low intensity). We select
10 multiprogrammed workloads, shown in Table~\ref{table:wklds}, for our
evaluations.

\begin{table}
\centering
\footnotesize{
\begin{tabular}{|l|l|l|}
\hline
\textbf{Mix} & \textbf{Workloads} & \textbf{Category} \\
\hline
\hline
WL-1 & mcf mcf mcf mcf & 4H \\
\hline
WL-2 & mcf lbm milc libquantum & 4H\\
\hline
WL-3 & libquantum mcf milc leslie3d & 4H  \\
\hline
WL-4 & milc leslie3d libquantum milc & 4H \\
\hline
WL-5 & libquantum milc astar wrf & 2H+2M\\
\hline
WL-6 & milc mcf soplex bwaves & 2H+2M \\
\hline
WL-7 & milc leslie3d GemsFDTD astar & 2H+2M \\
\hline
WL-8 & libquantum bwaves wrf astar& 1H+3M \\
\hline
WL-9 & bwaves wrf soplex GemsFDTD & 4M  \\
\hline
WL-10 & gcc gcc gcc gcc & 4L \\
\hline
\end{tabular}
}
\vspace{-0.05in}
\caption{Multiprogrammed workloads.}
\label{table:wklds}
\end{table}

\noindent\textbf{Evaluating the effect of dynamic power management:}
Ideally, we would like to run \emph{seconds}-long simulations to monitor
applications' working set sizes during the runtime and dynamically power
down/up banks as the working set sizes change throughout the simulation.
However, the simulation time would become prohibitively long with such an
approach. As a result, we decided to decouple the simulation and look at
different aspects of our dynamic power management framework separately.

First, we evaluate the steady-state system performance of different mapping
schemes when different numbers of banks are turned on. To do so, each simulation
is configured with a specific number of shutdown banks and is run for 500
million cycles. This allows us to examine system performance impact of
each mapping scheme's cacheline distribution under different
bank configurations.

Second, to evaluate the transition overhead of powering down or up banks, we
first warm up the DRAM cache with all banks enabled (power down) or the
specified number of banks disabled (power up). Once the warm-up completes, we
power down or up banks, and measure the latency of the transition.  For
transition evaluations, each simulation is run for 150 million warm-up cycles,
and 50 million execution cycles. The execution time is short because we only
need to collect statistics during the transition, and 50 million cycles are
long enough for the transition to complete.


'11110111', '11010111', '11010101', '10010101', '10010001', '10000001', '10000000'

\noindent\textbf{Performance Metrics:} We report system performance using the
\emph{System IPC}~\cite{multiprogram_metrics} metric: $\sum_{i=1}^N{IPC_{i}^{shared}}$.
In addition, we report the transition latency of powering up and down banks in
\emph{cycles}.



==> secs/seq.tex <==
\putsec{eval}{Experimental Evaluation}

\subsection{Steady-State Performance}

Shutting down DRAM cache banks results in different cacheline-to-bank mappings
depending on the scheme being used. Bank Fail-Over (BFO) can cause an imbalanced
distribution of cache lines to banks, as the fail-over banks tend to experience
higher capacity and conflict pressure. Modulo Re-Indexing (MRI) spreads
cache lines uniformly across the banks ensuring an even distribution over the
address space at the expense of requiring expensive remapping of all entries in
the cache.  In this work, we propose Cache Remapping Using Native Consistent Hashing
(CRUNCH) to achieve the best of both BFO and MRI, enabling fast transition
latency and balancing request load within the cache. We first examine the
load-balancing effect of each mapping scheme by observing the
\emph{steady-state} performance after banks are shutdown. \figref{steady.pdf}
shows the steady-state performance of each mapping scheme averaged across all
workloads for different numbers of active banks. We make several key
observations.

First, CRUNCH, with carefully designed region remapping tables, provides
performance comparable to MRI. In fact, except for three enabled banks, CRUNCH
provides slightly better average system performance than MRI. While MRI provides
even distribution over the address space, the simple \emph{modulo-k} mapping means
that accesses at strides that are not relatively prime to the number of enabled
banks will map to a restricted subset of the available banks.  In contrast, the RRT lookup
in CRUNCH performs a robust swizzling that will evenly distribute these strided accesses
across all available banks.  As a result, we expect that MRI coupled with a reasonable
swizzling scheme would perform on par with CRUNCH in the steady state.

Second, BFO considerably under-performs both CRUNCH and MRI when at least one
bank is powered down. BFO creates unbalanced load distribution by mapping all
the cache lines within a shutdown bank to the next available consecutive bank.
For instance, when one bank is shut down, one bank will receive roughly twice as much request
traffic as the other remaining banks. To quantitatively compare the load balancing effect
between different mapping schemes, we define a metric called the imbalance ratio.
The imbalance ratio is the maximum request traffic to any bank divided by the minimum
request traffic to any other bank.  With three powered-down banks, we observe the imbalance
ratios are 4.2, 1.3, and 1.0 for BFO, CRUNCH, and MRI, respectively, on average across all
workloads. The high bank imbalance leads BFO to reduce average system
performance by 11.6\% compared to CRUNCH.  Also note that the imbalance ratio for BFO is
a function of the specific banks shut down, allowing certain bank shutdown patterns to have much worse
imbalance than others.

CRUNCH provides the ability to consistently provide low imbalance ratios, enabling high system
performance, for all workloads.  Thus, we conclude that CRUNCH achieves the design goal
of load-balancing cache line distribution across banks.

\figputT{steady.pdf}{0in 0in 0in 0in}{Steady-state IPC performance of the
evaluated bank remapping schemes across varying numbers of enabled DRAM cache
banks. \% values are improvements of CRUNCH over MRI.}

%\kevin{using the putssec macro stops my vim-plugin spell check. We can always
%format section headers globally by changing jpaper.cls.}

\subsection{Power-Down Transition Latency}
Powering down a cache bank requires two phases of operation, although these phases may
be partially overlapped.  The first phase is searching the bank for all modified
blocks so that they can either be migrated to another bank or written back to
main memory. The second phase is actually performing the data transfer.  The shutdown latency
associated with performing these operations is a factor in system performance as well as
determining how responsive a power management scheme can be to short-term changes in workload behavior.
\figref{powerdown-all.pdf} shows the power-down transition latency averaged
across all evaluated workloads for shutting down different numbers of banks. As
the number of powered-down banks decreases, the transition latency also drops
for CRUNCH and BFO, whereas the transition latency remains approximately the same
for MRI. This is because CRUNCH and BFO only need to walk through and transfer
dirty cache lines in the shutdown banks. In contrast, MRI requires walking
through every single bank since \emph{all} cache lines are remapped across the
remaining active banks after banks are shut down.

\noindent\textbf{Effect of hierarchical dirty lines tracking:}
\figref{powerdown-all-hier.pdf} shows the transition latency after applying the
proposed hierarchical dirty lines tracking mechanism, called \hier for short.
The value on top of each data bar indicates \% latency reduction of using \hier
compared to the baseline mapping shown in \figref{powerdown-all.pdf}. Using
\hier provides consistent latency reductions for all workloads and variations of
powered-down bank counts, with maximum reductions of 10\%, 5\%, and 9\% for BFO,
CRUNCH, and MRI, respectively. Nevertheless, the majority of the transition latency
remains due to the overhead of dirty cache line migration. The migration
overhead is the most significant for MRI because it remaps every cache line's
bank index whenever banks are dynamically added or removed from the active bank
population.

\noindent\textbf{Transition impact on instantaneous performance:}
To gain a better sense of how the power-down transition impacts instantaneous
performance and system responsiveness, \figref{powerdown-perflog-light.pdf} and
\figref{powerdown-perflog-intense.pdf} show detailed performance traces sampled
over time for two representative workloads, \mbox{WL-1} and \mbox{WL-2}, respectively, when shutting down two
banks. The y-axis indicates the number of retired instructions during the last
sampling period (500K cycles). Several observations can be made from this data.

First, the system performance drops significantly regardless of the mapping
schemes used for both workloads. The main reason for the performance degradation
is that the two primary latency components, cache walk and dirty data
transfer, stop the DRAM cache from servicing memory requests during the
transition phase to guarantee correctness.

Second, MRI has a much larger transition latency than both BFO and CRUNCH. The
main reason is that MRI requires walking through the whole cache to enumerate
dirty cache lines due to the uniform redistribution of cache lines across all
active banks. In addition, MRI provides lower system performance during the
initial program phase after the completion of power-down transitions for both
\mbox{WL-1} and \mbox{WL-2}. For example, \figref{powerdown-perflog-light.pdf}
clearly shows that the retired instruction curve for MRI falls below BFO and
CRUNCH after the transition completes at the sample point 305. This occurs because
MRI re-shuffles clean cache lines' bank indices when banks are shutdown.
Therefore, most of the requests will result in misses during the program phase
after the completion of power-down transitions.

Third, the transition overhead for \mbox{WL-2} is greater than \mbox{WL-1}
simply because \mbox{WL-2} has a much larger quantity of dirty data, thus
requiring longer latency for transferring these dirty cache lines.

\figputT{powerdown-all.pdf}{0in 0in 0in 0in}{The power-down transition
latencies of mapping schemes for varied numbers of powered-down
banks.}

\figputT{powerdown-all-hier.pdf}{0in 0in 0in 0in}{The power-down transition
latencies for varied numbers of powered-down banks. Value on top of each bar
indicates \% latency reduction provided by hierarchical dirty lines tracking.}

%\figputT{powerdown-2banks.pdf}{0in 0in 0in 0in}{The latency of shutting down 2
%banks for all workloads using different mapping schemes. \todo{use this instead
%of perf over time?}}

\figputT{powerdown-perflog-light.pdf}{0in 0in 0in 0in}{Performance of WL-1
sampled over time.}
\figputT{powerdown-perflog-intense.pdf}{0in 0in 0in 0in}{Performance of WL-2
sampled over time.}

\subsection{Power-Up Transition Latency}
Powering a cache bank back up requires finding all of the modified cache lines that
previously would have mapped to this bank, but were displaced elsewhere. This requires
searching one or more banks, and then either repatriating those cache lines back
to this bank, or writing them back to main memory. \figref{powerup-all.pdf}
shows the power-up transition latency averaged across all evaluated
workloads for different mapping schemes along with our proposed hierarchical
dirty lines tracking mechanism. We make the following observations.

First, using BFO consistently provides lower transition latency for powering up
banks compared to both CRUNCH and BFO across all variations of powered-up bank
counts. As explained in \S\ref{sec:repatriate}, this is because BFO only needs to
search through certain active banks that contain failed-over cache lines.
Finding these active banks are straightforward since they are the next sequential active
bank(s) relative to the powering-up bank(s). On the other hand, both CRUNCH and MRI
require searching every active bank to find the displaced dirty cache lines. As a result, the latency of
reading every cache line in the active banks to find displaced dirty lines
dominates the transition latency for CRUNCH and MRI without using hierarchical
dirty cache line tracking.

Second, hierarchical dirty lines tracking reduces the transition latency
significantly for all mapping schemes with maximum reductions of 66.2\%, 69.3\%,
and 66.2\% for BFO, CRUNCH, and MRI, respectively. In particular, the benefit is
the greatest when powering up one bank for CRUNCH because it eliminates most of
the unnecessary reads for finding displaced dirty data. This does not occur for
MRI when powering up one bank because MRI has significantly more dirty cache lines
for migrations due to its shuffling effect on all cache lines.

Although BFO provides the lowest power-up transition latency among all the
mapping schemes, it has the disadvantage of leading to potential unbalanced
cache line distribution, causing some banks to become hot-spots forming a
bottleneck for memory requests to these banks. Therefore, BFO's lower power-up latency
comes at the cost of reduced steady-state system performance. In contrast, CRUNCH
not only provides high system performance with load-balancing distribution of cache lines, but also
enables fast transition latency for powering down banks and offers comparable
power-up transition latency as MRI. By applying a simple optimization,
hierarchical dirty lines tracking, the powered-up transition latency gap between
BFO and CRUNCH significantly reduces. In addition, with other optimizations that
can more efficiently enumerate dirty data or bound the amount of dirty data in
the cache, could further reduce the transition latency gap between BFO and
CRUNCH. Therefore, we conclude that CRUNCH achieves the
goals of enabling low transition latency and providing load-balanced cache line
distribution.

\figputT{powerup-all.pdf}{0in 0in 0in 0in}{The power-up transition
latencies of different bank mapping schemes averaged across all workloads
for turning on different numbers of banks.}

%\gabe{I'm thinking that for space reasons and because it may be similar to power-down, we might not
%need to show any examples of the detailed timing.  However, if it's much different (especially with
%the dirty-bits and/or xenophobic policy), it still might be worthwhile.  Depends on how tight we
%are on space.}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%To evaluate the power-up transition overhead, we first warm up the DRAM cache
%with the specified number of banks disabled. Once the warm-up terminates, those
%disabled banks are powered up. As a result, the amount of dirty data that need
%to be repatriated is proportional to the number of enabled banks during the
%warm-up.  In reality, the amount of \emph{displaced} dirty cachelines is actually
%bounded by the number of shutdown banks that migrated those dirty cachelines
%during the previous power-down transition.
%\kevin{I don't know if it makes sense to make a comparison between BFO and CRUNCH
%for this powerup experiment due to the reason above. The right way to do this
%is to power up banks after shutting down banks.}

%\figref{powerup-all.pdf} shows that the transition latency for MRI reduces as
%the number of powered up banks increases. However, BFO and CRUNCH do
%not follow the same trend. Their latency curves increase to a point, peaking at
%four powered-up banks, and drop as the bank count continues to increase.  To
%understand these trends, let us examine \figref{powerup-mig-lines.pdf}, which
%shows the number of migrated lines averaged across all workloads for different
%mapping schemes with varied number of powered up banks. As we can see, the
%trends for the latency curves follow the trends for the amount of migrated
%cachelines. The reason why migrated cachelines increase linearly for MRI is that
%MRI not only transfer displaced dirty cachelines to the powered up banks, but
%also transfer dirty cachelines between active banks since cachelines are
%uniformly redistributed across all banks when banks are dynamically powered up
%and down. On the other hand, the amount of migrated dirty cachelines is
%proportional to the number of powered-up banks until the point where the number
%of active banks becomes less than the number of powered-up banks since the
%amount of dirty data is bounded by the capacity of active banks. As a result,
%the number of dirty lines that need to be migrated maximizes at four enabled
%banks, thus having the maximum transition latency.

%\figputT{powerup-mig-lines.pdf}{0in 0in 0in 0in}{The power-up transition
%latencies of different bank mapping schemes averaged across all workloads
%for turning on different numbers of banks.}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Performance of Bank Utility Predictor}

In \S\ref{sec:bup}, we stated that the goal of our bank utility predictor (BUP)
is to achieve performance within 5\% of having all banks enabled.
\figref{predictor.pdf} shows the comparison between BUP's predicted number of
banks and the observed optimal numbers determined by exhaustive search for each
workload. In addition, \figref{bup-norm-ipc.pdf} shows the performance of each
workload with the predicted bank count, normalized to the all banks enabled case.

The data shows that BUP successfully predicts the exhaustively determined optimal value for half
of the workloads. The BUP scheme over-predicts the number of required banks for three workloads, which is
more acceptable behavior from the performance perspective, since the performance remains
within the 5\% target. However, BUP misses opportunities to reduce DRAM cache
power consumption in these cases. On the other hand, the BUP scheme under-predicts for WL-1 and WL-2,
which further reduces power consumption by \todo{X\% and Y\% compared to using the
optimal numbers at the cost of degrading performance by 10.8\% and 7.5\%,
respectively.}

We also observe that WL-10, which consists four copies of \texttt{gcc}, does
not benefit from using the DRAM cache, having less than 1\% performance degradation
without using the DRAM cache. This is because \texttt{gcc} has \emph{very low}
memory intensity (< 2 L3-MPKI).  Having extra cache capacity and bandwidth
provides minimal performance improvement for this workload.  Due to this observation, BUP
identifies very low memory-intensity application by monitoring applications'
MPKI values over time. If the total MPKI is less than a very low threshold, $5$
in our experiments, BUP makes the decision to shut down the entire DRAM cache.

%\todo{I think what we can do here is for each workload, run it once to see what the predicted
%number of banks to enable should be, then run it again with that number of banks statically
%enabled.  Then show the performance compared to having all banks enabled (ideally, we should be
%able to turn off quite a few banks with minimal performance impact).  Perhaps have another
%graph (or instead of performance) that just shows the ideal number of banks from the working-set
%size analysis, and then shows how many we predict.}

\figputT{predictor.pdf}{0in 0in 0in 0in}{Accuracy of the bank utility predictor.}
\figputT{bup-norm-ipc.pdf}{0in 0in 0in 0in}{System performance of the bank
utility predictor.}

\putssec{power}{Power Impact}
\todo{
\begin{itemize}
    \item Memory system power for different number of banks enabled?  This would include
    both DRAM cache (refresh and leakage reduction from shutting off banks)
    and main memory (to account for the extra traffic from increased misses).
    \item Energy required for transition (power-up or down).
\end{itemize}
}
Probably need two plots here.
%
\figputPlaceHolder{overallMemoryPower}{\todo{DRAM cache and main memory power (ideally) for varying number of
enabled banks.  Plus, mark the data point(s) corresponding to the number of banks that the predictor
says to enable.}}
%
\figputPlaceHolder{transitionEnergy}{\todo{Joules needed to power-down a bank for different schemes.  Perhaps
for power-up, too.}}

\subsection{Sensitivity Studies}
\todo{
\begin{itemize}
    \item Varying DRAM cache sizes?  Focus on transition times?  That's what'll be impacted the most
    because if the number of channels/banks remain the same, then the transition time will be impacted by
    having to walk more rows to check for dirty data to migrate, and there should be more total dirty data
    to migrate as well.  See \figref{cache-size-power-down}.
    \item Varying number of cores? May not have time for this.
    \item Alternative/even-more-naive BFO (sequentially shutting down banks)?  Show steady-state performance
    results only, as the transition times should be similar to the more balanced
    shut-down order. See \figref{steady-naive.pdf}.
    \item Some sort of characterization and/or visualization of bank-level load balancing?
    %See \figref{loadMap}.
\end{itemize}
}
%
\figputPlaceHolder{cache-size-power-down}{\todo{Power-down transition times for 256MB, 512MB and 1GB caches?}}

\figputT{steady-naive.pdf}{0in 0in 0in 0in}{Steady-state performance comparisons
between sequential- and balanced-order bank shutdown for BFO and CRUNCH. \%
values are performance degradations of BFO-SEQ relative to BFO.}

\figputPlaceHolder{loadMap}{\todo{Would be cool to simple collect the number of accesses per bank, and
sample this every, say, 1-5M cycles.  Run a simulation where you first turn off one bank, wait a while,
turn off another ank, wait a while, and so on.  For Consistent Hashing and MRI, the load should continually
be balanced across banks.  For BFO, we should see a non-uniform ``heat map'' develop.}}

%%%%%%%%%%%%%%%%%%%
\label{sec:naive-pattern}
\figref{steady-naive.pdf} shows the steady-state performance comparisons
between sequential and balanced bank shutdown orders. The value on top of each
group indicates \% performance difference between BFO-SEQ and BFO. We make the
following observations. First, BFO significantly reduces system performance when
banks are being turned off sequentially. This is because BFO creates an
unbalanced load distribution by mapping all the cachelines within the shutdown
banks to a single active bank. Second, CRUNCH provides the same system
performance compared to that of using balanced shutdown orders even if banks are
sequential disabled. This quantitatively demonstrates that CRUNCH provides a
robust and high-performance cacheline mapping scheme.


